Safe Control of Quadruped in Varying Dynamics via Safety Index Adaptation

Varying dynamics pose a fundamental difficulty when deploying safe control laws in the real world. Safety Index Synthesis (SIS) deeply relies on the system dynamics and once the dynamics change, the previously synthesized safety index becomes invalid. In this work, we show the real-time efficacy of Safety Index Adaptation (SIA) in varying dynamics. SIA enables real-time adaptation to the changing dynamics so that the adapted safe control law can still guarantee 1) forward invariance within a safe region and 2) finite time convergence to that safe region. This work employs SIA on a package-carrying quadruped robot, where the payload weight changes in real-time. SIA updates the safety index when the dynamics change, e.g., a change in payload weight, so that the quadruped can avoid obstacles while achieving its performance objectives. Numerical study provides theoretical guarantees for SIA and a series of hardware experiments demonstrate the effectiveness of SIA in real-world deployment in avoiding obstacles under varying dynamics.

==> sections/_introduction.tex <==
% [Paragraph 1] Short paragraph on how important provable safe control law is when deploying controllers in real-life applications. Then, end with a sentence on how important it is for safe controllers to adapt to changing dynamics.

% When deploying robots in real-life applications, it is crucial that certain safety constraints, such as collision avoidance, are always satisfied.
When deploying robots in real-life applications, maintaining safety constraints like collision avoidance is crucial.
Safe control has been widely studied to ensure constraint satisfaction for dynamic systems, with two representative approaches being the safe set algorithm (SSA) \cite{liu2014control} and control barrier functions (CBF) \cite{ames2014control}.
They quantify safety using energy functions and derive safe control laws that keep system states within a user-specified safe set, ensuring forward invariance (FI) \cite{chen2023safetyindexsynthesisstatedependent}, meaning the system stays in the safe region once entered.
% constrain system states within a safe set, defined as a level set of the energy function.
% Formally, such property is referred to as forward invariance (FI) \cite{chen2023safetyindexsynthesisstatedependent}, meaning that once the system lands in the safe region, it never leaves that region.
This property is sufficient to guarantee safety as long as the system is initially safe, which is usually the case.
% However, in practice, due to discretization errors and hardware noises, the system might still enter unsafe regions when it operates along the boundary of the safe set.
However, in practice, discretization errors and hardware noise may lead the system into unsafe areas when it operates near the boundary of the safe set.
% To mitigate that issue, we also desire the safe control law to bring the system back to safety in a finite time when it is outside safe regions.
To address this, the safe control law must also ensure finite-time convergence (FTC), bringing the system back to safety, as proved to be satisfied by SSA~\cite{chen2023safetyindexsynthesisstatedependent}.
% That additional property is referred to as finite time convergence (FTC), which has been proved to be satisfied by SSA \cite{chen2023safetyindexsynthesisstatedependent}.

% [Paragraph 2] Introduce SIS and the concepts of FI and FTC. Make this medium-length.

Although SSA provides strong theoretical guarantees, synthesizing a valid safe control law for an arbitrary constrained control problem is non-trivial.
% The most critical aspect is that for the safe control to ensure safety, it must always be feasible in the first place.
% Namely, at every state, some system input within the control limit must exist to satisfy the safe control constraints to make the safe control law realizable.
The most critical aspect is to ensure that, at every state, a control input within the limits exists to satisfy the safe control constraints to make the safe control law realizable. 
% This leads to infinite constraints since it should apply to any system state within the continuous state space.
% To solve that challenge, safety index synthesis \cite{chen2023safetyindexsynthesisstatedependent,zhao2022safety} has been proposed to construct feasible, safe control laws via sum-of-squares programming (SOSP).
To mitigate the issue of infinite constraints arising from this aspect in continuous state space, safety index synthesis (SIS)~\cite{chen2023safetyindexsynthesisstatedependent,zhao2022safety} has been developed, using sum-of-squares programming (SOSP) to construct feasible and safe control laws.

 \begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/pipeline_success.png}
    \caption{Trajectory of the quadruped carrying various packages of different weights (left column) and overall pipeline (right column). The quadruped avoids each obstacle sequentially, in the order of (1) blue, (2) green, and (3) red cubes, using safety index. Once the quadruped arrives at a goal position after avoiding an obstacle, a different package is loaded on its back. At this point, the safety index is adapted to the new dynamics.}
    \label{fig:full_traj}
\end{figure}

SIS provides a systematic way to construct provably safe control laws for constrained control problems.
Notably, the resulting safe control law is only valid for the specific system dynamics used for synthesis and may fail when the system dynamics change, which often occurs in real-life scenarios.
% For instance, when a quadrupedal robot follows a customer to carry groceries in a store, the robot dynamics might vary frequently when the customer adds or removes the payload.
% For instance, a quadruped robot's dynamics can shift when carrying varying payloads while assisting a customer in a store.
For instance, a shopping companion quadruped may experience various dynamic shifts as new payloads are placed on the back of the quadruped.
To maintain safety, the safe control law must adapt to these real-time changes in dynamics.
% In those cases, directly reapplying SIS for every new dynamics is impractical because solving SIS can take up to several minutes, even for simple dynamics.
Reapplying SIS for each new dynamics is impractical, as it can take several minutes to solve, even for simple dynamics.
% Instead of running full SIS for each dynamics variation, safety index adaptation (SIA) \cite{chen2024sia} has been proposed to adapt the safe control law to varying dynamics in a matter of seconds, significantly reducing the absence of safety guarantees caused by dynamics mismatch.
To handle this, safety index adaptation (SIA)~\cite{chen2024sia} has been proposed, allowing safe control laws to adapt to changing dynamics within seconds, significantly reducing the safety risks from mismatches in dynamics.

% [Paragraph 3] “Varying dynamics is really important, but not easy to deal with. SIA helps with that!” Here, we introduce SIA. 
% Important things to mention:
% How varying dynamics actually arises in the real-world when deploying robotic dogs. 
% → Quite simple: quadrupeds carrying packages or groceries.
% Why SIS is not something you can use in varying dynamics.
% → Simply takes too long.
% What is SIA’s edge on this issue:
% Fast adaptation time
% Allows varying dynamics AND varying control bounds (theoretically)
% Provides FI and FTC guarantees

% [Paragraph 4] Okay, SIA sounds amazing since it provides this and that! But have you tested this? THIS is where our work comes in!

The above line of safe control literature established a promising paradigm for provable safety.
However, these methods have only been validated in simulations with simple dynamics.
To ensure practical safety guarantees, verifying SIS and SIA on physical robots is necessary.
This paper demonstrates the effectiveness of SIA in changing real-world dynamics.
Specifically, we apply SIA to a quadruped robot that navigates to multiple goals while carrying varying payloads and avoiding obstacles.
% Despite the change in system dynamics, the adapted safety index provides safety guarantees for the quadruped when carrying its packages.
We demonstrate that SIA is essential to avoid failures (e.g., collision and losing balance) and fast enough for online safe control law adaptation.
To summarize, our contributions are:
% \begin{enumerate}
%     \item Guaranteed safety for real quadruped robots in navigation tasks with varying dynamics.
%     \item Comparison to non-adapted cases to validate the efficacy of safety index adaptation.
%     \item Comprehensive analysis of safety characteristics of adapted safety indices.
% \end{enumerate}
\begin{enumerate}
    \item We guarantee safety for real quadruped robots in navigation tasks with varying dynamics.
    \item We improve the efficiency of safety index adaptation and validate its efficacy in real life.
    \item We provide a comprehensive analysis of safety characteristics of adapted safety indices.
    \item We introduce a linear model for quadruped robots and a method to identify the varying dynamics.
\end{enumerate}

% Thus, fine-tuning the safety index parameters instead of generating a new one is an efficient method for adapting safe control laws in real robotic systems. 

% Safety has become one of the main interests in autonomous systems in recent years as more applications are deployed in the real world. In particular, safe control has gained much traction for its mathematical robustness in providing safety guarantees for autonomous systems. Energy functions~\cite{wei2019unified} in particular are widely used for safe control by mapping dangerous states to high values and safe states to low values, and ensuring safety by finding a safe control input that dissipates the energy. 



==> sections/_related_work.tex <==
% [Paragraph 1] SIS and safe control

% [Paragraph 2] Adaptive safe control

% [Paragraph 3] General quadruped carrying things, especially for safety, such as Tairan's paper.

In this section, we survey previous works on synthesis of safe controllers, adaptive safe controllers for varying dynamics, and synthesis of adaptive safe controllers. 
Furthermore, we briefly discuss existing work on deploying safe controllers on quadrupeds. 
We focus on energy-function-based safe controllers.

\textbf{Synthesis of Safe Controllers:} These studies focus on developing algorithmic approaches for synthesizing safe controllers. SIS has been studied extensively, with semidefinite programming playing a crucial role. For instance,~\cite{zhao2022safety} tackles SIS for known systems with control bounds, while~\cite{chen2023safetyindexsynthesisstatedependent} extends this to state-dependent control bounds. Additionally,~\cite{clark2022semi} leverages SOSP to synthesize various types of CBFs. In contrast, learning-based synthesis approaches~\cite{ma2022joint,liu2022inputsat,dawson2022safecontrollearnedcertificates,so2023trainneuralcontrolbarrier} have been explored, though they lack the mathematical rigor necessary for safety guarantees. Furthermore,~\cite{wei2022safe} utilizes an evolutionary method to synthesize safety indices for neural-network dynamic models.
% , while~\cite{wei2022persistently} employs convex semi-infinite programming to design uncertainty-robust safety indices.
 
\textbf{Adaptive Safe Controllers:} This body of work focuses on the theory of safe controllers under varying dynamics. There are two main paradigms in safe control under such dynamics: \textit{robust} safe controller aims to provide safety under bounded uncertainties~\cite{xu2015rCBF,jankovic2018robust} and \textit{adaptive} safe controller estimates the changes in the dynamics~\cite{ames2020aCBF}. The intersection of these two, \textit{robust-adaptive} safe controller, has also been studied~\cite{lopez2023unmatched}. Adaptive safe controllers are less conservative compared to robust safe controllers since they do not consider the ``worst-case" scenarios.

\textbf{Synthesis of Adaptive Safe Controllers:} This category is concerned with developing algorithmic approaches for synthesizing adaptive safe controllers. Although SIS for constant dynamics has been studied extensively, synthesis of adaptive safe controllers under changing dynamics has not been studied widely to our knowledge. The closest is~\cite{sliu2024racbf}, which synthesizes a robust-adaptive CBF (raCBF) using SOSP. On the other hand, there are some works done in adapting safe controllers online to changing dynamics.~\cite{maghenem2021adaptiveSafety} introduces a hybrid adaptive law for CBFs, but only tests its controller in a 2-dimensional simulation.~\cite{chen2024sia} leverages Sylvester's criterion to readily adapt safety index to varying dynamics and provides the central theory and methodology for our work.

\textbf{Safe Control of Quadrupeds:} These works involve deploying energy-function-based safe controllers on quadruped platforms in real life. While some work exists in deploying CBFs~\cite{liao2023walkingnarrowspacessafetycritical}, we are unaware of any previous work deploying adaptive safe controllers on quadruped hardware.


==> sections/conclusion.tex <==
% 1. only 2d
% 2. dt needs much improvement
% 3. analysis of SIA in local search space
% 4. analysis of hardware
